Stackable and queueable permutations

There is a natural bijection between permutations obtainable using a stack (those avoiding the pattern 312) and permutations obtainable using a queue (those avoiding 321). This bijection is equivalent to one described by Simion and Schmidt in 1985. We argue that this bijection might well have been found back in 1968 by readers of volume 1 of Knuth's *The Art of Computer Programming*, if Knuth had not assigned difficulty ratings to his exercises.

==> knuth_dot_bib <==
@article {claesson,
    AUTHOR = {Claesson, Anders and Kitaev, Sergey},
     TITLE = {Classification of bijections between 321- and 132-avoiding
              permutations},
   JOURNAL = {S\'em. Lothar. Combin.},
  FJOURNAL = {S\'eminaire Lotharingien de Combinatoire},
    VOLUME = {60},
      YEAR = {2008},
     PAGES = {Article B60d},
eprint = {arXiv:0805.1325v1 [math.CO]},
}
@article {richards:knuth,
    AUTHOR = {Richards, Dana},
     TITLE = {Ballot sequences and restricted permutations},
   JOURNAL = {Ars Combin.},
  FJOURNAL = {Ars Combinatoria},
    VOLUME = {25},
      YEAR = {1988},
     PAGES = {83--86},
}
@book {knuth:vol1first,
    AUTHOR = {Knuth, Donald E.},
     TITLE = {The art of computer programming. {V}olume 1: {F}undamental algorithms},
 PUBLISHER = {Addison-Wesley},
EDITION={First},
      YEAR = {1968},
}
@book {knuth:vol1second,
    AUTHOR = {Knuth, Donald E.},
     TITLE = {The art of computer programming. {V}olume 1: {F}undamental algorithms},
   EDITION = {Second},
 PUBLISHER = {Addison-Wesley},
      YEAR = {1973},
}
@book {knuth:vol3,
    AUTHOR = {Knuth, Donald E.},
     TITLE = {The art of computer programming. {V}olume 3: {S}orting and searching},
 PUBLISHER = {Addison-Wesley},
EDITION={First},
      YEAR = {1973},
}
@article {simionschmidt,
    AUTHOR = {Simion, Rodica and Schmidt, Frank W.},
     TITLE = {Restricted permutations},
   JOURNAL = {European J. Combin.},
  FJOURNAL = {European Journal of Combinatorics},
    VOLUME = {6},
      YEAR = {1985},
    NUMBER = {4},
     PAGES = {383--406},
}
@article {rt:dek,
    AUTHOR = {Rosenstiehl, Pierre and Tarjan, Robert E.},
     TITLE = {Gauss codes, planar {H}amiltonian graphs, and stack-sortable
              permutations},
   JOURNAL = {J. Algorithms},
  FJOURNAL = {Journal of Algorithms},
    VOLUME = {5},
      YEAR = {1984},
    NUMBER = {3},
     PAGES = {375--390},
}
@article {bona:survey,
    AUTHOR = {B{\'o}na, Mikl{\'o}s},
     TITLE = {A survey of stack-sorting disciplines},
      NOTE = {Permutation patterns (Otago, 2003)},
   JOURNAL = {Electron. J. Combin.},
  FJOURNAL = {Electronic Journal of Combinatorics},
    VOLUME = {9},
      YEAR = {2002/03},
    NUMBER = {2},
     PAGES = {Article 1, 16},
       URL = {http://www.combinatorics.org/Volume_9/Abstracts/v9i2a1.html},
}
@incollection {pratt:dek,
    AUTHOR = {Pratt, Vaughan R.},
     TITLE = {Computing permutations with double-ended queues, parallel
              stacks and parallel queues},
 BOOKTITLE = {Fifth {A}nnual {ACM} {S}ymposium on {T}heory of {C}omputing
              ({A}ustin, {T}ex., 1973)},
     PAGES = {268--277},
 PUBLISHER = {Assoc. Comput. Mach., New York},
      YEAR = {1973},
}
@article {west:twostack,
    AUTHOR = {West, Julian},
     TITLE = {Sorting twice through a stack},
      NOTE = {Conference on Formal Power Series and Algebraic Combinatorics
              (Bordeaux, 1991)},
   JOURNAL = {Theoret. Comput. Sci.},
  FJOURNAL = {Theoretical Computer Science},
    VOLUME = {117},
      YEAR = {1993},
    NUMBER = {1-2},
     PAGES = {303--313},
       DOI = {10.1016/0304-3975(93)90321-J},
       URL = {http://dx.doi.org/10.1016/0304-3975(93)90321-J},
}
@article {zeilberger:twostack,
    AUTHOR = {Zeilberger, Doron},
     TITLE = {A proof of {J}ulian {W}est's conjecture that the number of
              two-stack-sortable permutations of length {$n$} is
              {$2(3n)!/((n+1)!(2n+1)!)$}},
   JOURNAL = {Discrete Math.},
  FJOURNAL = {Discrete Mathematics},
    VOLUME = {102},
      YEAR = {1992},
    NUMBER = {1},
     PAGES = {85--93},
       DOI = {10.1016/0012-365X(92)90351-F},
       URL = {http://dx.doi.org/10.1016/0012-365X(92)90351-F},
}
@article {tarjan:networks,
    AUTHOR = {Tarjan, Robert},
     TITLE = {Sorting using networks of queues and stacks},
   JOURNAL = {J. Assoc. Comput. Mach.},
  FJOURNAL = {Journal of the Association for Computing Machinery},
    VOLUME = {19},
      YEAR = {1972},
     PAGES = {341--346},
}
@book{kitaev:patterns,
AUTHOR={Kitaev, Sergey},
Title={Patterns in Permutations and Words},
YEAR={2011},
PUBLISHER={Springer}
}
@incollection {evenitai,
    AUTHOR = {Even, S. and Itai, A.},
     TITLE = {Queues, stacks, and graphs},
 BOOKTITLE = {Theory of machines and computations ({P}roc. {I}nternat.
              {S}ympos., {T}echnion, {H}aifa, 1971)},
     PAGES = {71--86},
 PUBLISHER = {Academic Press},
      YEAR = {1971},
}
@incollection {unger:88,
    AUTHOR = {Unger, Walter},
     TITLE = {On the {$k$}-colouring of circle-graphs},
 BOOKTITLE = {S{TACS} 88},
    SERIES = {Lecture Notes in Comput. Sci.},
    VOLUME = {294},
     PAGES = {61--72},
 PUBLISHER = {Springer},
      YEAR = {1988},
       DOI = {10.1007/BFb0035832},
       URL = {http://dx.doi.org/10.1007/BFb0035832},
}
@incollection {unger:92,
   author = {Unger, Walter},
   title = {The complexity of colouring circle graphs},
   booktitle = {S{TACS} 92},
   series = {Lecture Notes in Comput. Sci.},
   publisher = {Springer},
   pages = {389-400},
   volume = {577},
   url = {http://dx.doi.org/10.1007/3-540-55210-3\_199},
   doi = {10.1007/3-540-55210-3\_199},
   year = {1992}
}

